Towards a Sentiment-Aware Conversational Agent

In this paper, we propose an end-to-end sentiment-aware conversational agent based on two models: a reply sentiment prediction model, which leverages the context of the dialogue to predict an appropriate sentiment for the agent to express in its reply; and a text generation model, which is conditioned on the predicted sentiment and the context of the dialogue, to produce a reply that is both context and sentiment appropriate. Additionally, we propose to use a sentiment classification model to evaluate the sentiment expressed by the agent during the development of the model. This allows us to evaluate the agent in an automatic way. Both automatic and human evaluation results show that explicitly guiding the text generation model with a pre-defined set of sentences leads to clear improvements, both regarding the expressed sentiment and the quality of the generated text.

==> bibliography.tex <==
% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
\bibliography{bibliography.bib}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)
%\begin{thebibliography}{1}
%\bibitem{IEEEhowto:kopka}
%H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
%  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.
%\end{thebibliography}

==> text_generation.tex <==
\section{Text Generation}
\label{chap:text-generation}

In this work we are proposing to develop a customer support sentiment-aware conversational agent. Traditionally, state-of-the-art dialogue conversational agents rely on large amounts of conversational data to train text generation models, which are able to generate human-like responses, both regarding the context of the conversation, and having lexical diversity \cite{zhang2020dialogpt}. In particular, \cite{rashkin2019towards}, shows that state-of-the-art text generation models can be fine-tuned with appropriate dialogue empathetic data, and express emotions. However, when there is not enough data available, these approaches might lead to models which are unable to implicitly generate text with the aforementioned characteristics. Our goal is to develop a system which is able to have those characteristics, in particular, by taking advantage of explicit sentiment information.

In Chapter \ref{chap:sentiment-analysis} we proposed two models that can be part of a guided dialogue text generation pipeline, which allow to understand the sentiment of the context sentences, and predict the appropriate sentiment that should be expressed next. What is left is to describe the text generation model we are going to use in order to incorporate the sentiment information.
During a dialogue, this model will receive the sentiment predicted by the reply sentiment prediction model. Then, it will use this information, as well as the previous context of the conversation, to generate a sentence that is not only appropriate given a context, but that expresses the predicted sentiment.

In this chapter we will begin by describing the base model (Section \ref{section:tg-baseline}). We will make use of pre-trained Transformer language models, such as the GPT-2 \cite{radford2019language}, which have been shown to provide strong baselines for text generation. Next, we will describe how we will improve upon the baseline. In particular, we are going to adapt the work by \cite{wolf2019transfertransfo}, which proposes a model that is able to leverage a set of sentences that describe a given persona in order to generate text that is coherent with the persona. We will adapt this concept and develop a sentiment lexicon knowledge base, which will be used to make the conversational agent sentiment-aware (Section \ref{section:tg-guide-model}). In addition to this, we will also describe how we are going to adapt the next sentence prediction approach, proposed by \cite{devlin2019bert} and used to fine-tune the model proposed by \cite{wolf2019transfertransfo}, through the use of distractors, for our specific use-case (Section \ref{section:tg-next-sentence-pred}).

% #############################################################################
\subsection{Base Model}
\label{section:tg-baseline}
In Section \ref{subsection:text-generation-GPT}, we described one of the current state-of-the-art text generation architectures, the Generative Pre-trained Transformer (GPT), which has had three iterations: GPT-1 \cite{radford2018improving}, GPT-2 \cite{radford2019language}, and GPT-3 \cite{brown2020language}. Since the original GPT-3 model is still not publicly avaiable, and due to the computational costs of similar implementations \cite{gpt-neo} we will use the GPT-2 model for our work. In this section we will describe in more detail the GPT-2 architecture, and explain how it is used for dialogue text generation.

In Figure \ref{fig:tg-base-model}, we can observe the input and output of the GPT-2 model. In order to make a language model such as the GPT-2 suitable for the dialogue task, as described in \cite{wolf2019transfertransfo}, we concatenate previous context of the dialogue (history) to the input of the model. This is possible by introducing two extra special tokens to the model, \texttt{<speaker1>}, which indicates the beginning of a sequence from the user, and \texttt{<speaker2>}, which indicates the beginning of a sequence from the bot, in addition to the existing special tokens \texttt{<BOS>}, which indicates the beginning of a sequence, \texttt{<EOS>}, which indicates the end of a sequence. Furthermore, in this figure we can also see the autoregressive property of this model. As described in Section \ref{subsection:autoregressive-lm}, autoregressive language models use the left-wise context of a sentence in order to calculate the probability of the next word. This means that this model uses previously generated words as input to generate new ones. At each timestep $t$, the input of the model is $\textsc{concat}(h;w_{0:t-1})$, with $h$ representing the history, and $w_{0:t-1}$ representing a sequence of generated words from timestep $0$ until $t-1$. The output is $w_t$, which is the word generated at timestep $t$.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\columnwidth]{Images/gpt2.png}
    \caption{Example of the input and output of the base GPT-2 model adapted for the dialogue task.}
    \label{fig:tg-base-model}
\end{figure}

\subsection{Condition Model with Sentiment}
\label{section:tg-guide-model}
In order to condition the text generation base model with a desired sentiment, we follow the work of \cite{wolf2019transfertransfo} which proposes two increments to the base model: the first, at the input level, where sentences that describe a persona are concatenated to the input of the model; and the second, at the fine-tuning level, which uses a double-head Transformer model for multi-task learning that jointly fine-tunes the model for two tasks, language modelling (the original task) and next sentence prediction. The next sentence prediction task, proposed by \cite{devlin2019bert}, is implemented in this work through the use of distractors. To do so, between two and six randomly selected sentences (distractors) for each example in the corpus are concatenated to that input's history, creating two to six extra examples. The goal of the next sentence prediction head is to classify whether the sentence appended to the input is correct. In this section we will describe how we are going to adapt these two approaches to build a generation model that is conditioned on a given sentiment.

\subsubsection{Adding Sentiment Lexicon}
\label{subsection:sentiment-lexicon}

We will start by improving the base model by introducing information from a knowledge base in order to guide the generation. Instead of a persona, we will input lexicon that represents the desired sentiment. This is done by concatenating the lexicon to the beginning of the input of the model. An advantage of this model is that we can experiment with various sentiment lexicons, which can consist of a single word for each sentiment (for example, the name of the sentiment), expressions, or full sentences. In Figure \ref{fig:tg-sentiment} we illustrate how concatenating sentiment lexicon to the input of the GPT-2 model might guide the generation model to output a sentence that expresses the desired sentiment. For instance, by adding the sentiment lexicon of the \textit{anger} emotion, we expect the model to produce a more sentiment appropriate sentence (\say{I am annoyed}), than the base model (\say{Fine, thank you}), given the same history. 

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\columnwidth]{Images/gpt2-sentiment.pdf}
    \caption{Example of the input and output of the sentiment controlled GPT-2 model through the concatenation of sentiment lexicon to the input of the model.}
    \label{fig:tg-sentiment}
\end{figure}



\subsubsection{Next Sentence Prediction}
\label{section:tg-next-sentence-pred}

The work by \cite{wolf2019transfertransfo} also describes a training particularity regarding the loss that is calculated to update the weights of the model. The model used is called a double head Transformer and is trained for two different tasks. First, the language model head, is tasked with generating the tokens, from which a language model loss is calculated. Second, the next sentence prediction head, task proposed in \cite{devlin2019bert}, is evaluating whether the reply is appropriate given a history and a sentiment lexicon. From this task, a next sentence prediction loss is calculated. Then, the model's weights are updated conditioned on the weighted sum of the language model loss, and the next sentence prediction loss, $\mathcal{L} = \alpha \mathcal{L}_{\text{LM}} + \beta \mathcal{L}_{\text{NSP}}$, with $\mathcal{L}$ representing the total loss, $\mathcal{L}_{\text{LM}}$, the loss of the language model, $\mathcal{L}_{\text{NSP}}$, the loss of the next sentence prediction model, and $\alpha$ and $\beta$ the weights given to each of the losses.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\columnwidth]{Images/gpt2-distractors.pdf}
    \caption{Example of the training of the double head transformer. The first head, the language model head, is tasked with generating a reply given a history and the sentiment lexicon. The second head, the next sentence prediction head, given four similar inputs but with different reply possibilities (the gold and the distractors) is tasked with classifying whether they are appropriate given the sentiment lexicon and the history.}
    \label{fig:tg-distractors}
\end{figure}

The next sentence prediction task is trained through the use of distractors, as exemplified in Figure \ref{tab:tg-distractors}. During training, the model is not only learning to generate sentences, but also to classify whether the provided training sentences are appropriate given the history and the desired sentiment. The goal of this architecture is to teach the model which sentences are appropriate to answer, but in particular, which are not. To do so, in addition to the gold example, which includes the sentiment lexicon, history, and the gold reply, we also provide the model three additional examples, where instead of concatenating the gold reply, we concatenate a random sentence from the training set that is labelled with a different sentiment than the one the model is supposed to generate. For example, in Figure \ref{fig:tg-distractors}, the goal is to generate the sentence \say{I am annoyed}, which expresses the \textit{anger} sentiment. As distractors, we use three sentences labelled with the sentiments \textit{joy}, \textit{fear}, and \textit{sadness}.

\subsection{Summary}
Having the reply sentiment prediction model as a way to inform the text generation model of the appropriate reply emotion, we proposed a text generation model that is able to leverage this information to condition its output on the desired sentiment.
In particular, we adapted the work by \cite{wolf2019transfertransfo}, that is able to express a given persona, to our use-case. We started by introducing the base model, which uses four new special tokens in order to make the text generation model suitable for the dialogue task. Next, we saw how we can concatenate sentiment lexicon to the input of the model in order to guide it towards the desired sentiment. Finally, we adapted the next sentence prediction task, with the use of sentiment distractors, as a way to teach the model which sentences are not appropriate to answer given the desired sentiment and a history.
